Quantum Robustness Verification: A Hybrid Quantum-Classical Neural Network Certification Algorithm

In recent years, quantum computers and algorithms have made significant progress indicating the prospective importance of quantum computing (QC). Especially combinatorial optimization has gained a lot of attention as an application field for near-term quantum computers, both by using gate-based QC via the Quantum Approximate Optimization Algorithm and by quantum annealing using the Ising model. However, demonstrating an advantage over classical methods in real-world applications remains an active area of research. In this work, we investigate the robustness verification of ReLU networks, which involves solving a many-variable mixed-integer programs (MIPs), as a practical application. Classically, complete verification techniques struggle with large networks as the combinatorial space grows exponentially, implying that realistic networks are difficult to be verified by classical methods. To alleviate this issue, we propose to use QC for neural network verification and introduce a hybrid quantum procedure to compute provable certificates. By applying Benders decomposition, we split the MIP into a quadratic unconstrained binary optimization and a linear program which are solved by quantum and classical computers, respectively. We further improve existing hybrid methods based on the Benders decomposition by reducing the overall number of iterations and placing a limit on the maximum number of qubits required. We show that, in a simulated environment, our certificate is sound, and provide bounds on the minimum number of qubits necessary to approximate the problem. Finally, we evaluate our method within simulation and on quantum hardware.

==> results.tex <==
\section{Results}\label{sec:results}

\textbf{Architecture, Dataset and Training Methods.} We conduct experiments with one type of multilayer perceptron (MLP) neural network: MLP-$2\text{x}[20]$. Here MLP-$m\text{x}[n]$ refers to $m$ hidden layers and $n$ units per hidden layer. The network uses ReLU functions after every fully connected layer. We train our model on the MNIST dataset for $20$ epochs with a batch size of $128$ in two ways: (i) with a regular loss function and (ii) adversarially trained via the Projected Gradient Descent (PGD) as in \citet{madry2017towards}. In case of a regularly trained model, we keep the name MLP-$2\text{x}[20]$, while we refer to it as PGD-$2\text{x}[20]$ if it is adversarially trained. The clean accuracy on test set for the different networks are $95,62\%$ and $86,73\%$ for MLP-$2\text{x}[20]$ and PGD-$2\text{x}[20]$, respectively. The adversarial training used adversarial examples from the infinity norm ball around the input with radius $\epsilon = 0.01$. 

\textbf{Experimental Setup.} We divide the hardware into classical and quantum computing. On the classical side, we ran the algorithm on a server having 4xCPUs Intel(R) Xeon(R) E7-8867 v4 running at 2.40GHz for a total of 72/144 cores/threads. On the quantum side, we used two different system types: quantum annealing and gate-based quantum computers. In the first case, we access the D-Wave Advantage\textsuperscript{TM} system 5.1 constructed with 5760 qubits in two ways: (i) directly on the Quantum Processing Unit (QPU) and (ii) with the Hybrid solver provided by D-Wave Leap\footnote{D-Wave Leap\textsuperscript{TM} Quantum Cloud Service https://cloud.dwavesys.com/leap/}, which makes use of a Tabu search to further decompose the problem and run a part on the QPU. In the second case, we used the QAOA\footnote{Python library Qiskit v0.36.0 https://github.com/Qiskit/qiskit} runtime program of the IBMQ\footnote{IBM Quantum https://quantum-computing.ibm.com/} cloud on the IBM Brooklyn QC having the Hummingbird r2 architecture of 65 qubits, a quantum volume of 32, and 1.5K circuit layers operations per second.

\subsection{Evaluation of Robustness}

We compare our method against a complete (\textbf{Exact})~\cite{tjeng2018evaluating} and incomplete (\textbf{Convex})~\cite{wong2018provable} verifier with the MIP formulation as in \autoref{eq:general_verification} and the convex relaxation from \autoref{eq:convex_relaxation}.
We evaluate the empirical performance of HQ-CRAN in an ideal setting, i.e. where the \textit{master} and \textit{sub} problems are solved using the IBM ILOG CPLEX\footnote{IBM (2020) IBM ILOG CPLEX 20.1 User’s Manual (IBM ILOG CPLEX Division, Incline Village, NV)} software on a classical computer.
For a fair comparison, we propagate the boundaries through the network with interval arithmetic for all methods, and evaluate all methods on the first 100 samples from the MNIST test set with $\epsilon\in\{\frac{1}{255},\frac{2}{255},\frac{4}{255},\frac{8}{255}\}$ as adversarial budget. We use HQ-CRAN with the improvements of \autoref{sec:improvements} and real variables for $\eta$ and $a_k$. 
%
\begin{table}[ht!]
\captionsetup{font=small}
\caption{
Adversarial robustness of MNIST classifiers to perturbations of $\epsilon$ in a $l_\infty$-norm. 
We run each algorithm on the first 100 test set samples from the MNIST dataset. 
The times are expressed in seconds.
}
\label{table:robustness}
\vskip -0.05in
\begin{footnotesize}
\begin{sc}
\resizebox{\columnwidth}{!}{%

\begin{tabular}{lccccccc}
\toprule
Network &$\epsilon$ &\multicolumn{3}{c}{Certified Accuracy $\uparrow$} &\multicolumn{3}{c}{Average Time [s]$\downarrow$} \\
                    &                    & Exact &HQ-CRAN &Convex &Exact &HQ-CRAN &Convex \\
\midrule
PGD-$2\text{x}[20]$& $\nicefrac{1}{255}$  &$88\%$ &$88\%$ &$88\%$ &$0.04$ &$0.31$ &$0.004$ \\
                    & $\nicefrac{2}{255}$ &$88\%$ &$88\%$ &$88\%$ &$0.06$ &$0.36$ &$0.004$ \\
                    & $\nicefrac{4}{255}$ &$88\%$ &$85\%$ &$85\%$ &$0.10$ &$0.61$ &$0.005$ \\
                    & $\nicefrac{8}{255}$ &$81\%$ &$81\%$ &$61\%$ &$0.13$ &$1.10$ &$0.006$ \\
\midrule
MLP-$2\text{x}[20]$& $\nicefrac{1}{255}$   &$96\%$ &$96\%$   &$96\%$ &$0.05$ &$0.42$ &$0.005$ \\
                    & $\nicefrac{2}{255}$  &$96\%$ &$95\%$  &$95\%$ &$0.07$ &$0.62$ &$0.005$ \\
                    & $\nicefrac{4}{255}$  &$95\%$ &$95\%$  &$95\%$ &$0.10$ &$1.04$ &$0.005$  \\
                    & $\nicefrac{8}{255}$  &$80\%$ &$73\%$  &$24\%$ &$0.14$ &$9.39$ &$0.006$ \\
\bottomrule
\end{tabular}}
\end{sc}
\end{footnotesize}
% \vskip -0.1in
\end{table}

In terms of final robustness certification, we report in Table~\ref{table:robustness} the certified accuracy, i.e., the fraction of verified and correctly classified samples of all test samples. 
To limit the compute time, we set the maximum number of iterations $T$ to 500 and the target gap $\xi$ between the \textit{master} and \textit{sub} problem to $1$. 
Within these settings, HQ-CRAN behaves similarly to \textbf{Convex} up to an $\epsilon$ of $\nicefrac{4}{255}$, and shows better results for $\nicefrac{8}{255}$. 
As previously presented in~\autoref{sec:method}, our method places itself in the middle of \textit{complete} and \textit{incomplete} verification methods. 
The outer approximation of \textbf{Convex} demonstrates poor performances for $\epsilon = \nicefrac{8}{255}$, indicating that outer approximations struggle to verify larger perturbations.
\tom{use beta-crown. if we dont manage to do it here. then we should at least say that there are more advanced approximation techniques}
On the contrary, our average runtime is $\sim2$ orders of magnitude slower than \textbf{Convex}. As this work is only a proof-of-concept and it is expected that the algorithm is slower than both the \textbf{Exact} and \textbf{Convex}, we do not consider current state-of-the-art verifiers based on GPUs, such as $\beta$-CROWN \cite{wang2021betacrown} or GPUPoly \cite{mueller2021scaling}
\tom{+ we should probably include the timings + I dont know the term augmented perturbations}

\subsection{Simulations in Classical Computing}
%
\begin{figure}[htb!]
\vskip -0.2in
\begin{center}
\includegraphics[width=\columnwidth]{plots/v1_v2.pdf}
\captionsetup{font=small}
\caption{
    Optimality ratio between the certified lower bounds of HQ-CRAN, without~(\textbf{v1}) and with~(\textbf{v2}) improvements, and the exact values of \textbf{Exact}. 
    In the context of HQ-CRAN, the bounds for the sub problem and the maximum number of iterations $T$ have been set to $500$. 
    The gap $\xi$ has been set to $1$. 
    We report the distribution as interquartile range of the first 100 samples of the MNIST test set on PGD-$2\text{x}[20]$.
    }
\label{fig:real_pgd}
\end{center}
\vskip -0.3in
\end{figure}
%
We further conduct evaluations on our improvements presented in \autoref{sec:improvements}. 
For this reason, we structure it as an ablation study and to distinguish the approaches, we define two versions of HQ-CRAN. 
The first version (\textbf{v1}) can be seen as a baseline as it is similar to the earlier proposed algorithm of \cite{chang2020quantum}, which lacks the \textit{additional} problem of \autoref{eq:additional_problem} and the Hamming distance. Instead the second version (\textbf{v2}) uses both. 
All versions compute the minimum number of qubits with Corollaries~\ref{cor:p} and~\ref{corr:a_x}.
We start the experiments with a comparison of the final objective values for each inner minimization of \autoref{eq:general_verification}. 
For a fair evaluation, we compare our results in terms of \textit{optimality ratio} between the final master objective $m_t$ and the solution $m^*$ of \textbf{Exact}, defined as:
%
\begin{equation*}
    R = \left\{ 
    \begin{aligned}
        &\nicefrac{m^*}{m_t}                     &&\text{if} \; m_t > 0, \\
        &\nicefrac{m_t}{m^*}                     &&\text{else if} \; m^* < 0, \\
        &\nicefrac{m^*}{\left(m^* - m_t\right)}  &&\text{elsewhere.}
    \end{aligned}
    \right.
\end{equation*}
%
In \autoref{fig:real_pgd}, we show the comparison in terms of optimality ratio, average number of iterations and average time per class. In the context of \textbf{v2}, the results demonstrate a clear reduction on the average number of iterations and time while maintaining a high optimality ratio. These advantages are even more significant for larger $\epsilon$ values. Overall, in both methods the average optimality ratio remains very close to 1. The maximum size of the cuts set $\varphi$ has been set to infinity, i.e. all cuts are considered.


\begin{table*}[htbp]
\captionsetup{font=small}
\caption{Comparison between simulated and quantum annealing on the \textit{master} of HQCRAN, without \textbf{v1} and with \textbf{v2} improvements. The maximum number of iterations $T$ has been set to $15$ and the gap $\xi$ to $1$ and the \textit{sub} problem boundaries $\overline{\vectsym{\alpha}}$ and $\overline{\vectsym{\beta}}$ to $5$. The penalty weights $w_a$ and $w_p$ were set to 0.1 and 0.01, respectively. The maximum size of the cuts set $\varphi$ has been set to infinity and $5$ for \textbf{v1} and \textbf{v2}, respectively. We run each algorithm on the first 100 samples of the MNIST test set.}
\begin{minipage}{\linewidth}
\begin{center}
\begin{footnotesize}
\begin{sc}
\begin{tabular}{cccccccccccccc}
\toprule
\multirow{3}{*}{Networks} & \multirow{3}{*}{$\epsilon$} &\multicolumn{4}{c}{Correct Solutions $\uparrow$} &\multicolumn{4}{c}{Average \# Iterations $\downarrow$} &\multicolumn{4}{c}{Average \# of Qubits $\downarrow$} \\
&  &\multicolumn{2}{c}{Simulated} &\multicolumn{2}{c}{Quantum} &\multicolumn{2}{c}{Simulated} &\multicolumn{2}{c}{Quantum} &\multicolumn{2}{c}{Simulated} &\multicolumn{2}{c}{Quantum} \\
& &\multicolumn{1}{c}{v1} &\multicolumn{1}{c}{v2} &\multicolumn{1}{c}{v1} &\multicolumn{1}{c}{v2} &\multicolumn{1}{c}{v1} &\multicolumn{1}{c}{v2} &\multicolumn{1}{c}{v1} &\multicolumn{1}{c}{v2} &\multicolumn{1}{c}{v1} &\multicolumn{1}{c}{v2} &\multicolumn{1}{c}{v1} &\multicolumn{1}{c}{v2} \\
\midrule
\multirow{4}{*}{PGD-$2$x$[20]$}
&$\nicefrac{1}{255}$ &$94\%$    &$96\%$  &$74\%$  &$73\%$ &$4\pm2$ &$3\pm2$     &$4\pm3$ &$3\pm2$   &$59\pm35$  &$45\pm21$  &$52\pm45$ &$37\pm17$ \\
&$\nicefrac{2}{255}$ &$82\%$    &$91\%$  &$54\%$  &$50\%$ &$6\pm3$ &$4\pm3$     &$4\pm3$ &$3\pm2$   &$82\pm43$  &$58\pm23$  &$65\pm48$ &$46\pm20$ \\
&$\nicefrac{4}{255}$ &$52\%$    &$67\%$  &$36\%$  &$34\%$ &$8\pm3$ &$7\pm4$    &$5\pm4$  &$5\pm3$   &$121\pm50$ &$77\pm20$  &$80\pm54$ &$59\pm21$ \\
&$\nicefrac{8}{255}$ &$10\%$    &$17\%$    &$13\%$   &$11\%$  &$12\pm3$ &$11\pm4$   &$9\pm5$  &$7\pm4$   &$186\pm44$ &$94\pm10$   &$139\pm70$   &$81\pm19$ \\
\midrule
\multirow{4}{*}{MLP-$2$x$[20]$} 
&$\nicefrac{1}{255}$ &$83\%$    &$85\%$ &$65\%$ &$61\%$     &$6\pm3$    &$5\pm3$    &$5\pm4$ &$4\pm2$ &$88\pm47$  &$64\pm22$ &$77\pm53$ &$52\pm20$ \\
&$\nicefrac{2}{255}$ &$61\%$    &$65\%$ &$38\%$ &$37\%$     &$8\pm3$    &$7\pm4$    &$5\pm4$ &$5\pm4$ &$112\pm51$ &$75\pm20$ &$80\pm54$ &$60\pm21$  \\
&$\nicefrac{4}{255}$ &$27\%$    &$30\%$ &$17\%$ &$17\%$     &$10\pm4$   &$10\pm4$    &$6\pm4$ &$7\pm5$ &$155\pm56$ &$88\pm15$ &$93\pm61$ &$72\pm24$ \\
&$\nicefrac{8}{255}$ &$3\%$     &$4\%$  &$4\%$ &$6\%$     &$14\pm2$   &$14\pm2$   &$12\pm5$ &$10\pm5$ &$214\pm30$ &$100\pm5$ &$179\pm66$ &$93\pm16$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{footnotesize}
\end{center}
\end{minipage}
\label{tab:annealing}
\end{table*}


\subsection{Quantum Hardware Experiments}

We continue our evaluation with a comparison between simulated\footnote{Python dwave-neal v0.5.7, general Ising graph simulated annealing solver.} and quantum annealing. 
Embedding the problem into a QA requires solving the minor embedding problem. 
In our case, we use the clique embedding strategy \cite{boothby2016fast} which handle the connectivity problem in a way that each connection larger than the maximum available size (in case of Advantage it is $\sim$15) is handled with long chains between qubits. 
To decrease the chains, before submitting the model to the sampler, we prune connections below a certain threshold (5$\%$) and retaining only interactions with values commensurate with the sampler’s precision. In both simulated and quantum annealing, the number of reads was set to 100 and in the context of simulated annealing, the number of sweeps was set to 50000.

In \autoref{tab:annealing}, we report the numerical results in terms of percentage of correct solutions, i.e. solutions where $m_t \leq m^*$. 
The average number of qubits reflects the size of the \textit{master} problem before being embedded into the quantum hardware. 
We notice that the number of correct solutions decrease for increased values of $\epsilon$. The behaviour has to be attribute to the maximum number of iterations $T$ fixed to $15$. 
This choice limits the convergence of the algorithm but gives us a fair comparison between the approaches. 
As previously mentioned, the limiting factor is the clique embedding which fixes the maximum size of logical qubits to $177$ on the Advantage~\cite{mcgeoch2021advantage}. 
The \textbf{v2} shows an overall reduced number of qubits with respect to \textbf{v1} while maintaining approximately the same correctness. 
\tom{I would extract the settings here. It is a bit hard to read still. Go maybe like this: in the quantum experiment we use chain ... logical qubits ... max iterations ...  and then: In table 2 we can see the results and we see that v2 performs... I think this will make it better and is basically how you did it before}\\

Finally, we evaluate HQ-CRAN running on a gate-based quantum computer via QAOA and on a quantum annealer via Leap.
Due to time limits on the quantum hardware, we present results on the first and the first ten MNIST test set samples for QAOA and Leap, respectively.
This also restricts our hyperpameter choices for QAOA to the Perturbation Stochastic Approximation optimizer with a maximum iteration number of 10 instead of 100, 2 repetitions and 1024 shots. 
For Leap we use the default 3-minute execution time limit.
The penalty weights $w_a$ and $w_p$ were set to 0.1 and 0.01, respectively. $\epsilon=\frac{1}{255}$ and a target gap $\xi$ of 1 for both algorithms.
With this setting, QAOA starts of with $\sim28$ qubits and requires 13 additional qubits per step.
For Leap, the number of theoretical qubits is identical but one needs to add qubits required for increased connectivity as discussed previously.


\begin{figure}[t]
\captionsetup{font=small}
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{plots/hardware_comparison.pdf}}
\caption{Average and standard deviation of the difference between \textit{master} and \textit{sub} objective at each iteration for QAOA and Leap. In the case of Leap, we plot the first 10 samples of the MNIST test set. In contrast, for QAOA, we only show the first one. We used an $\epsilon$ value of $\nicefrac{1}{255}$ and PGD-$2\text{x}[20]$.}
\label{fig:hardware_steps}
\end{center}
\vskip -0.3in
\end{figure}

\autoref{fig:hardware_steps} shows the convergence behavior of Leap and QAOA.
The gap is defined as difference between the objectives of \textit{master} and \textit{sub} problems at each iteration. The solution is reached when the gap is lower than our target gap $\xi=1$.
While we find QAOA not converging by the constrained accessibility and limitations of current QC hardware, Leap converges close to the optimal solution within 6 steps for all tested samples.

==> sections/additional_material.tex <==


In the first case, we access the hybrid solver from D-Wave Leap cloud, which embeds a part of the problem into the advantage system 5.1 constructed with 5760 qubits. In the second case, we used the QAOA runtime program of the IBMQ cloud on the IBM Brooklyn QC having the Hummingbird r2 architecture of 65 qubits and a quantum volume of 32.

\textbf{Solvers.}
We tested \textit{HQ-CRAN} with different solvers for the master problem of \autoref{eq:qubo}:
\begin{itemize}
    \itemsep-0.3em 
    \item Classic Computing
    \begin{enumerate}
        \item \textbf{Real}: IBM ILOG CPLEX\footnote{IBM (2020) IBM ILOG CPLEX 20.1 User’s Manual (IBM ILOG CPLEX Division, Incline Village, NV)} solver with real objective $p$ and real artificial variables. %\todo{should be better described?}
        \item \textbf{Anneal}: Simulated annealing\footnote{D-Wave-Neal 0.5.9 simulated annealing sampler.} algorithm. A Probabilistic technique for approximating the global optimum.
    \end{enumerate}
    \item Quantum Computing
    \begin{enumerate}
        \item \textbf{QAOA}: QAOA runtime algorithm implemented on gate-based quantum computer.
        \item \textbf{Leap}: D-Wave Leap hybrid algorithm which further decomposes and embeds the problem into a Quantum Annealing processing unit.
    \end{enumerate}
\end{itemize}





\begin{table*}[htbp]
\captionsetup{font=scriptsize}
\caption{Hybrid Benders decomposition applied to the robustness verification of neural networks. We use real variables for $p$ and $a_k$ and CPLEX to solve both master and sub problems. The maximum number of iterations has been set to $500$ and the gap to $1$. We run each algorithm on the first 100 samples of the MNIST dataset. The average time is per class.}
\begin{center}
\begin{footnotesize}
\begin{sc}
%
\begin{tabular}{lcccccccc|}
\toprule
\multirow{2}{*}{Networks} & \multirow{2}{*}{$\epsilon$} &\multicolumn{2}{c}{Optimality Ratio $\uparrow$} &\multicolumn{2}{c}{\# Iterations $\downarrow$} &\multicolumn{2}{c}{Time [sec.]} \\
&  &v1 &v2 &v1 &v2 &v1 &v2 \\
\midrule
\multirow{4}{*}{PGD-$2$x$[20]$} 
&$\nicefrac{1}{255}$ &$0.94\pm0.04$ &$0.94\pm0.04$     &$4\pm2$ &$3\pm1$           &$0.34$ &$0.31$ \\
&$\nicefrac{2}{255}$ &$0.93\pm0.05$ &$0.93\pm0.05$     &$6\pm2$ &$4\pm1$           &$0.52$ &$0.36$ \\
&$\nicefrac{4}{255}$ &$0.91\pm0.12$ &$0.92\pm0.08$     &$10\pm9$ &$6\pm18$         &$1.14$ &$0.61$ \\
&$\nicefrac{8}{255}$ &$0.85\pm0.56$ &$0.87\pm0.44$     &$27\pm25$ &$9\pm5$         &$4.26$ &$1.10$ \\
\midrule
\multirow{4}{*}{MLP-$2$x$[20]$} 
&$\nicefrac{1}{255}$ &$0.95\pm0.03$ &$0.95\pm0.03$      &$5\pm3$    &$4\pm2$        &$0.38$   &$0.33$  \\
&$\nicefrac{2}{255}$ &$0.94\pm0.04$ &$0.94\pm0.04$      &$8\pm5$    &$6\pm18$         &$0.64$  &$0.54$  \\
&$\nicefrac{4}{255}$ &$0.91\pm0.08$ &$0.92\pm0.07$      &$16\pm15$  &$8\pm5$          &$1.70$  &$0.72$  \\
&$\nicefrac{8}{255}$ &$0.83\pm0.45$ &$0.86\pm0.26$      &$58\pm60$  &$19\pm16$        &$14.50$ &$2.43$  \\
\bottomrule
\end{tabular}
\end{sc}
\end{footnotesize}
\label{tab:improvements}
\end{center}
\end{table*}
